Monetary Incentives, Landowner Preferences: Estimating Cross-Elasticities in Farmland Conversion to Renewable Energy

This study examines the impact of monetary factors on the conversion of farmland to renewable energy generation, specifically solar and wind, in the context of expanding U.S. energy production. We propose a new econometric method that accounts for the diverse circumstances of landowners, including their unordered alternative land use options, non-monetary benefits from farming, and the influence of local regulations. We demonstrate that identifying the cross elasticity of landowners' farming income in relation to the conversion of farmland to renewable energy requires an understanding of their preferences. By utilizing county legislation that we assume to be shaped by land-use preferences, we estimate the cross-elasticities of farming income. Our findings indicate that monetary incentives may only influence landowners' decisions in areas with potential for future residential development, underscoring the importance of considering both preferences and regulatory contexts.

==> commondefs <==
#
# Rules and definitions for building various things, especially 
# TeX documents.
# -- Andrew Myers
# Last updated April 2007
#

MAKEDIR = .
INCLDIR = .
TEXDIR = .

COMMONRULES = $(MAKEDIR)/commonrules

SOURCES = $(CFILES) $(C++FILES) $(YFILES) $(LFILES) $(AFILES)
OBJECTS = $(CFILES:.c=.o) $(C++FILES:.C=.o)
DIRT = *.o core *.aux *.dvi *.log *.stamp *.i *.bbl *.[ib]lg $(LDIRT)
GENERATED = .dependtime Makedepend Makedepend.bak
RM = rm -f
MKDEPFILE = Makedepend
MKDEPEND = makedepend
MKDEPFLAGS = -Y
MKDEPC++FLAGS = $(C++DEFS) $(C++INCS) $(MKDEPFLAGS)
MKDEPCFLAGS = $(CDEFS) $(CINCS) $(MKDEPFLAGS)

.SUFFIXES: .C .ps .i .txt .h
.SUFFIXES: .tex .dvi .ind .idx .bbl .aux .glo .aux .stamp .pdf .eps

GNUBIN = /usr/local

ATTC++ = CC
DECC++ = cxx
GNUC++ = g++

CC = cc
C++ = $(GNUC++)
YACC = bison
DVIPS = dvips

C++F = $(C++) $(C++FLAGS)
CCF = $(CC) $(CFLAGS)

C++FLAGS = $(C++OPTS) $(C++DEFS) $(C++INCS)

C++INCS = $(GC++INCS) $(LC++INCS)
C++OPTS = $(GC++OPTS) $(LC++OPTS)
C++DEFS = $(GC++DEFS) $(LC++DEFS)

GC++OPTS = $(OPTIMIZER)

CFLAGS = $(COPTS) $(CDEFS) $(CINCS)
COPTS = $(GCOPTS) $(LCOPTS)
CDEFS = $(GCDEFS) $(LCDEFS)
CINCS = $(GCINCS) $(LCINCS)

GCOPTS = $(OPTIMIZER)

M3F = $(M3) $(M3FLAGS)
M3 = m3
M3PP = m3pp

LDFLAGS = $(LLDFLAGS) $(GLDFLAGS)
LLDFLAGS = $(LLDLIBS) $(LLDOPTS) 

SEP=:
#SEP=\;         # for MikTeX+Cygwin
TEXINPUTS = .$(SEP)$(TEXDIR)$(SEP)
LATEX = TEXINPUTS=$(TEXINPUTS) latex
PDFLATEX = TEXINPUTS=$(TEXINPUTS) pdflatex


==> commonrules <==
# Some basic recursive rules for building, installing, and cleaning up
# a source tree
#
subdirs:
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make); \
	fi; done;

clean:  localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

localclean:
	$(RM) $(DIRT)

clobber: localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;
	$(RM) $(TARGETS) $(GENERATED)

install: default localinstall
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

incdepend: .dependtime
depend: .dependtime

.dependtime: $(SOURCES)
	touch temp
	$(MKDEPEND) $(MKDEPC++FLAGS) -f temp $(C++FILES)
	touch $(MKDEPFILE)
	$(MKDEPEND) $(MKDEPCFLAGS) -f $(MKDEPFILE) $(CFILES)
	cat temp >> $(MKDEPFILE)
	rm -f temp
	touch $@

# Rules for TeX files
#
# The line that runs LATEX needs to run inside a subshell to turn off
# "make"'s status checking. It blows away .aux because the .aux file
# created is bad and also breaks bibtex. It touches .stamp to force a
# rebuild.
.tex.dvi:
	@if test -r "$*.aux"; \
	   then cp $*.aux $*.auxprev; \
	   else echo > $*.auxprev; \
	fi
	@echo "$(LATEX) $<"
	@sh -c "$(LATEX) $< || (rm -f $*.aux; sleep 1; touch $*.stamp; exit 1)"
	@-cmp -s $*.aux $*.auxprev; \
	if test $$? = 1; \
	then \
	    sleep 1; \
	    echo "==> Rebuilding $@"; \
	    touch $*.stamp; \
	    $(MAKE) $@; \
	else \
	    echo "==> No need to rebuild $@"; \
	fi
	@rm -f $*.auxprev

.tex.pdf:
	@if test -r "$*.aux"; \
	   then cp $*.aux $*.auxprev; \
	   else echo > $*.auxprev; \
	fi
	@echo "$(PDFLATEX) $<"
	@sh -c "$(PDFLATEX) $< || (rm -f $*.aux; sleep 1; touch $*.stamp; exit 1)"
	@-cmp -s $*.aux $*.auxprev; \
	if test $$? = 1; \
	then \
	    sleep 1; \
	    echo "==> Rebuilding $@"; \
	    touch $*.stamp; \
	    $(MAKE) $@; \
	else \
	    echo "==> No need to rebuild $@"; \
	fi
	@rm -f $*.auxprev

# must add dependencies like
#    foo.ind: foo.stamp
#    foo.dvi: foo.ind
# to use this rule properly.
.tex.ind:
	@if [ -f $*.idx ]; then \
	   echo makeindex $*.idx; \
	   makeindex $*.idx; \
	else \
	   echo touch $@; \
	   touch $@; \
        fi

# must add dependencies like
#    foo.bbl: foo.bib
#    foo.dvi: foo.bbl
# to use this rule properly.
.tex.bbl:
	@if [ -r $*.aux ]; then echo bibtex $*; sh -c "bibtex $(BIBOPTS) $* || echo"; else echo; fi

.tex.stamp: # backward compatibility
	touch $@

.dvi.ps:
	$(DVIPS) $(DVIPSOPTS) $< -o $@
.eps.pdf:
	epstopdf $<

#
# Rules for C++ and .i files
#

.C.i:
	$(C++F) -E $< > $@

.c.i:
	$(CCF) -E $< > $@

.C.o:
	$(C++F) -c $<

# include $(M3SU)    # old Modula-3 rules


==> extensive_wind_w_rank.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Cross Return Elasticity of Farming and Solar and Wind Adoption}
\begin{tabular}{l*{7}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         &\multicolumn{1}{c}{(6)}         &\multicolumn{1}{c}{(7)}         \\
\midrule
Farm Return         &      -0.343\sym{**} &      -2.344\sym{**} &      -0.550         &       2.060         &      -0.846\sym{***}&      -0.066         &      -0.934         \\
                    &     (0.167)         &     (1.192)         &     (0.376)         &     (1.450)         &     (0.232)         &     (0.164)         &     (1.407)         \\
\addlinespace
Median Census Age   &      -0.021\sym{***}&      -0.033         &      -0.060\sym{***}&      -0.027         &       0.006         &       0.005         &       0.036         \\
                    &     (0.006)         &     (0.026)         &     (0.014)         &     (0.025)         &     (0.019)         &     (0.022)         &     (0.037)         \\
\addlinespace
Unemployment Rate   &       0.011\sym{**} &       0.015         &       0.018         &       0.002         &       0.023\sym{*}  &      -0.006         &       0.002         \\
                    &     (0.005)         &     (0.019)         &     (0.012)         &     (0.022)         &     (0.013)         &     (0.011)         &     (0.024)         \\
\addlinespace
ln\_gdp              &       0.100\sym{***}&       0.329\sym{**} &       0.134\sym{**} &       0.230\sym{***}&      -0.041         &      -0.038         &      -0.039         \\
                    &     (0.027)         &     (0.157)         &     (0.057)         &     (0.083)         &     (0.081)         &     (0.065)         &     (0.108)         \\
\addlinespace
ln\_lforce           &      -0.519\sym{***}&       0.421         &      -0.308         &      -0.308         &       0.230         &      -0.441         &       0.237         \\
                    &     (0.110)         &     (0.609)         &     (0.273)         &     (0.565)         &     (0.319)         &     (0.274)         &     (0.373)         \\
\addlinespace
Constant            &       6.834\sym{***}&       7.196         &       6.934\sym{*}  &     -12.475         &       3.115         &       5.751\sym{*}  &       2.640         \\
                    &     (1.480)         &     (5.261)         &     (4.080)         &    (13.457)         &     (2.872)         &     (3.050)         &     (7.270)         \\
\midrule
Obs.                &    3958.000         &     859.000         &     828.000         &     863.000         &     475.000         &     489.000         &     444.000         \\
County Fixed Effects&         yes         &         yes         &         yes         &         yes         &         yes         &         yes         &         yes         \\
Year Fixed Effects  &         yes         &         yes         &         yes         &         yes         &         yes         &         yes         &         yes         \\
R^2                 &       0.728         &       0.454         &       0.774         &       0.575         &       0.845         &       0.830         &       0.777         \\
\bottomrule
\multicolumn{8}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{8}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.010\)}\\
\end{tabular}
\end{table}


==> tables/extensive_both_wo_rank.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Cross Return Elasticity of Farming and Solar and Wind Adoption}\label{tab:both_wo_rank}
\begin{tabular}{l*{5}{c}}
\toprule
                    &\multicolumn{1}{c}{}         &\multicolumn{2}{c}{Extensive Margin}         &\multicolumn{2}{c}{Intensive Margin}  \\
                    &\multicolumn{1}{c}{First Stage IV}         &\multicolumn{1}{c}{Solar}         &\multicolumn{1}{c}{Wind}         &\multicolumn{1}{c}{Solar}         &\multicolumn{1}{c}{Wind}         \\
\midrule
High Heat Days      &      -0.006\sym{***}&                     &                     &                     &                     \\
                    &     (0.001)         &                     &                     &                     &                     \\
\addlinespace
Farm Return         &                     &      -0.132         &      -0.286\sym{*}  &      -0.171         &      -0.719         \\
                    &                     &     (0.184)         &     (0.168)         &     (0.535)         &     (1.163)         \\
\addlinespace
Median Census Age   &       0.002         &       0.032\sym{***}&      -0.022\sym{***}&       0.048\sym{**} &      -0.030         \\
                    &     (0.004)         &     (0.007)         &     (0.006)         &     (0.021)         &     (0.045)         \\
\addlinespace
Unemployment Rate   &       0.004         &       0.034\sym{***}&       0.010\sym{**} &       0.048\sym{***}&      -0.059\sym{*}  \\
                    &     (0.003)         &     (0.005)         &     (0.005)         &     (0.016)         &     (0.034)         \\
\addlinespace
Constant            &       6.324\sym{***}&      -0.718         &       2.621\sym{**} &      -1.127         &       6.041         \\
                    &     (0.167)         &     (1.183)         &     (1.078)         &     (3.434)         &     (7.459)         \\
\midrule
Obs.                &    3958.000         &    3958.000         &    3958.000         &    3958.000         &    3958.000         \\
County Fixed Effects&         yes         &         yes         &         yes         &         yes         &         yes         \\
Year Fixed Effects  &         yes         &         yes         &         yes         &         yes         &         yes         \\
$R^2$                 &       0.907         &       0.717         &       0.728         &       0.185         &       0.218         \\
\bottomrule
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{6}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.010\)}\\
\end{tabular}
\end{table}


==> tables/extensive_inv_mills.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Probability of Adoption of Wind and Solar with Power Transmission Lines}
\begin{tabular}{l*{2}{c}}
\toprule
                    &\multicolumn{1}{c}{Solar}         &\multicolumn{1}{c}{Wind}         \\
\midrule
main                &                     &                     \\
Median Census Age   &      -0.072\sym{***}&      -0.001         \\
                    &     (0.008)         &     (0.008)         \\
\addlinespace
Unemployment Rate   &       0.092\sym{***}&      -0.227\sym{***}\\
                    &     (0.022)         &     (0.025)         \\
\addlinespace
Number of Power Transmission Lines&       0.035\sym{***}&      -0.038\sym{***}\\
                    &     (0.005)         &     (0.006)         \\
\addlinespace
Power Transmission Voltage&      -0.000\sym{***}&       0.000\sym{***}\\
                    &     (0.000)         &     (0.000)         \\
\addlinespace
Constant            &       0.242         &      -0.733\sym{**} \\
                    &     (0.335)         &     (0.360)         \\
\midrule

\midrule
Obs.                &    3958.000         &    3958.000         \\
Year Fixed Effects  &         yes         &         yes         \\
$R^2$                 &                     &                     \\
\bottomrule
\multicolumn{3}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.010\)}\\
\end{tabular}
\end{table}


==> tables/extensive_solar_w_rank.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Cross Return Elasticity of Farming and Solar Adoption (Extensive Margin)}\label{tab:ext_sol_w_rank}
\begin{tabular}{l*{7}{c}}
\toprule
                    &\multicolumn{1}{c}{All}         &\multicolumn{3}{c}{Agriculture Ranked First}         &\multicolumn{3}{c}{Residential Ranked First}  \\
                                        &\multicolumn{1}{c}{}         &\multicolumn{6}{c}{Second Ranking Land Use}  \\
                    &\multicolumn{1}{c}{}         &\multicolumn{1}{c}{Solar}         &\multicolumn{1}{c}{Wind}         &\multicolumn{1}{c}{Residential}         &\multicolumn{1}{c}{Ag}         &\multicolumn{1}{c}{Solar}         &\multicolumn{1}{c}{Wind}         \\
\midrule
Farm Return         &      -0.132         &       1.486         &      -0.583         &      -0.680         &      -1.006\sym{**} &       0.154         &      -0.122         \\
                    &     (0.184)         &     (1.094)         &     (0.369)         &     (0.897)         &     (0.404)         &     (0.257)         &     (1.905)         \\
\addlinespace
Median Census Age   &       0.032\sym{***}&       0.024         &       0.003         &       0.032\sym{*}  &       0.095\sym{***}&       0.024         &       0.091\sym{*}  \\
                    &     (0.007)         &     (0.021)         &     (0.014)         &     (0.016)         &     (0.032)         &     (0.035)         &     (0.052)         \\
\addlinespace
Unemployment Rate   &       0.034\sym{***}&       0.035\sym{**} &       0.004         &       0.037\sym{**} &       0.094\sym{***}&       0.030\sym{*}  &       0.048         \\
                    &     (0.005)         &     (0.014)         &     (0.012)         &     (0.014)         &     (0.022)         &     (0.018)         &     (0.032)         \\
\addlinespace
Constant            &      -0.718         &     -10.870         &       3.469         &       2.761         &       3.502         &      -1.404         &      -2.165         \\
                    &     (1.183)         &     (7.673)         &     (2.346)         &     (5.352)         &     (2.871)         &     (1.853)         &    (11.041)         \\
\midrule
Obs.                &    3958.000         &     859.000         &     828.000         &     863.000         &     475.000         &     489.000         &     444.000         \\
County Fixed Effects&         yes         &         yes         &         yes         &         yes         &         yes         &         yes         &         yes         \\
Year Fixed Effects  &         yes         &         yes         &         yes         &         yes         &         yes         &         yes         &         yes         \\
$R^2$                 &       0.717         &       0.644         &       0.725         &       0.765         &       0.754         &       0.793         &       0.800         \\
\bottomrule
\multicolumn{8}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{8}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.010\)}\\
\end{tabular}
\end{table}


==> tables/extensive_wind_w_rank.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Cross Return Elasticity of Farming and Solar and Wind Adoption}\label{tab:ext_wind_w_rank}
\begin{tabular}{l*{7}{c}}
\toprule
                    &\multicolumn{1}{c}{All}         &\multicolumn{3}{c}{Agriculture Ranked First}         &\multicolumn{3}{c}{Residential Ranked First}  \\
                                        &\multicolumn{1}{c}{}         &\multicolumn{6}{c}{Second Ranking Land Use}  \\
                    &\multicolumn{1}{c}{}         &\multicolumn{1}{c}{Solar}         &\multicolumn{1}{c}{Wind}         &\multicolumn{1}{c}{Residential}         &\multicolumn{1}{c}{Ag}         &\multicolumn{1}{c}{Solar}         &\multicolumn{1}{c}{Wind}         \\
\midrule
Farm Return         &      -0.343\sym{**} &      -2.344\sym{**} &      -0.550         &       2.060         &      -0.846\sym{***}&      -0.066         &      -0.934         \\
                    &     (0.167)         &     (1.192)         &     (0.376)         &     (1.450)         &     (0.232)         &     (0.164)         &     (1.407)         \\
\addlinespace
Median Census Age   &      -0.021\sym{***}&      -0.033         &      -0.060\sym{***}&      -0.027         &       0.006         &       0.005         &       0.036         \\
                    &     (0.006)         &     (0.026)         &     (0.014)         &     (0.025)         &     (0.019)         &     (0.022)         &     (0.037)         \\
\addlinespace
Unemployment Rate   &       0.011\sym{**} &       0.015         &       0.018         &       0.002         &       0.023\sym{*}  &      -0.006         &       0.002         \\
                    &     (0.005)         &     (0.019)         &     (0.012)         &     (0.022)         &     (0.013)         &     (0.011)         &     (0.024)         \\
\addlinespace
ln\_gdp              &       0.100\sym{***}&       0.329\sym{**} &       0.134\sym{**} &       0.230\sym{***}&      -0.041         &      -0.038         &      -0.039         \\
                    &     (0.027)         &     (0.157)         &     (0.057)         &     (0.083)         &     (0.081)         &     (0.065)         &     (0.108)         \\
\addlinespace
ln\_lforce           &      -0.519\sym{***}&       0.421         &      -0.308         &      -0.308         &       0.230         &      -0.441         &       0.237         \\
                    &     (0.110)         &     (0.609)         &     (0.273)         &     (0.565)         &     (0.319)         &     (0.274)         &     (0.373)         \\
\addlinespace
Constant            &       6.834\sym{***}&       7.196         &       6.934\sym{*}  &     -12.475         &       3.115         &       5.751\sym{*}  &       2.640         \\
                    &     (1.480)         &     (5.261)         &     (4.080)         &    (13.457)         &     (2.872)         &     (3.050)         &     (7.270)         \\
\midrule
Obs.                &    3958.000         &     859.000         &     828.000         &     863.000         &     475.000         &     489.000         &     444.000         \\
County Fixed Effects&         yes         &         yes         &         yes         &         yes         &         yes         &         yes         &         yes         \\
Year Fixed Effects  &         yes         &         yes         &         yes         &         yes         &         yes         &         yes         &         yes         \\
$R^2$                 &       0.728         &       0.454         &       0.774         &       0.575         &       0.845         &       0.830         &       0.777         \\
\bottomrule
\multicolumn{8}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{8}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.010\)}\\
\end{tabular}
\end{table}


==> tables/intensive_solar_w_rank.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Cross Return Elasticity of Farming and Solar Adoption (Intensive Margin)}
\begin{tabular}{l*{7}{c}}
\toprule
                    &\multicolumn{1}{c}{All}         &\multicolumn{3}{c}{Agriculture Ranked First}         &\multicolumn{3}{c}{Residential Ranked First}  \\
                                        &\multicolumn{1}{c}{}         &\multicolumn{6}{c}{Second Ranking Land Use}  \\
                    &\multicolumn{1}{c}{}         &\multicolumn{1}{c}{Solar}         &\multicolumn{1}{c}{Wind}         &\multicolumn{1}{c}{Residential}         &\multicolumn{1}{c}{Ag}         &\multicolumn{1}{c}{Solar}         &\multicolumn{1}{c}{Wind}         \\
\midrule
Farm Return         &      -0.376\sym{**} &       0.035         &      -0.490         &      -0.460         &      -1.262         &      -0.648         &      -0.173         \\
                    &     (0.186)         &     (0.312)         &     (0.736)         &     (0.445)         &     (2.419)         &     (3.485)         &     (0.411)         \\
\addlinespace
Median Census Age   &       0.071\sym{**} &       0.021         &       0.094         &       0.001         &       0.478         &       0.278         &      -0.007         \\
                    &     (0.033)         &     (0.035)         &     (0.073)         &     (0.040)         &     (0.896)         &     (1.305)         &     (0.163)         \\
\addlinespace
Unemployment Rate   &       0.016         &       0.039         &      -0.006         &      -0.031         &       0.034         &       0.047         &       0.046         \\
                    &     (0.012)         &     (0.031)         &     (0.043)         &     (0.049)         &     (0.036)         &     (0.054)         &     (0.053)         \\
\addlinespace
Inverse Mills Ratio &       0.740\sym{***}&       0.671\sym{***}&       0.961\sym{***}&       0.583\sym{***}&       0.725\sym{***}&       0.962\sym{***}&       0.850\sym{***}\\
                    &     (0.051)         &     (0.148)         &     (0.241)         &     (0.171)         &     (0.199)         &     (0.253)         &     (0.177)         \\
\addlinespace
Constant            &      -0.276         &      -1.154         &      -0.279         &       3.344         &     -13.680         &      -3.679         &       1.427         \\
                    &     (0.918)         &     (2.115)         &     (4.157)         &     (3.241)         &    (25.270)         &    (17.937)         &     (3.259)         \\
\midrule
Obs.                &    3958.000         &     859.000         &     828.000         &     863.000         &     475.000         &     489.000         &     444.000         \\
County Fixed Effects&         yes         &         yes         &         yes         &         yes         &         yes         &         yes         &         yes         \\
$R^2$                 &       0.292         &       0.463         &       0.520         &       0.407         &       0.310         &       0.460         &       0.490         \\
\bottomrule
\multicolumn{8}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{8}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.010\)}\\
\end{tabular}
\end{table}


==> tables/intensive_wind_w_rank.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Cross Return Elasticity of Farming and Solar and Wind Adoption}
\begin{tabular}{l*{7}{c}}
\toprule
                    &\multicolumn{1}{c}{All}         &\multicolumn{3}{c}{Agriculture Ranked First}         &\multicolumn{3}{c}{Residential Ranked First}  \\
                                        &\multicolumn{1}{c}{}         &\multicolumn{6}{c}{Second Ranking Land Use}  \\
                    &\multicolumn{1}{c}{}         &\multicolumn{1}{c}{Solar}         &\multicolumn{1}{c}{Wind}         &\multicolumn{1}{c}{Residential}         &\multicolumn{1}{c}{Ag}         &\multicolumn{1}{c}{Solar}         &\multicolumn{1}{c}{Wind}         \\
\midrule
Farm Return         &      -0.939\sym{**} &      -1.120         &      -1.000         &      -1.436         &      -1.601         &       1.496         &       0.069         \\
                    &     (0.412)         &     (1.250)         &     (1.474)         &     (1.061)         &     (2.267)         &     (3.709)         &     (0.278)         \\
\addlinespace
Median Census Age   &       0.142\sym{*}  &      -0.100         &       0.139         &       0.313\sym{*}  &       0.516         &      -0.613         &       0.009         \\
                    &     (0.076)         &     (0.194)         &     (0.201)         &     (0.167)         &     (0.855)         &     (1.402)         &     (0.150)         \\
\addlinespace
Unemployment Rate   &      -0.030         &      -0.066         &       0.003         &      -0.073         &      -0.012         &      -0.027         &      -0.009         \\
                    &     (0.023)         &     (0.081)         &     (0.098)         &     (0.100)         &     (0.045)         &     (0.055)         &     (0.028)         \\
\addlinespace
Inverse Mills Ratio &       1.424\sym{***}&       1.706\sym{***}&       1.452\sym{***}&       1.409\sym{***}&       0.336         &       1.574\sym{*}  &       1.756\sym{**} \\
                    &     (0.120)         &     (0.391)         &     (0.417)         &     (0.339)         &     (0.364)         &     (0.878)         &     (0.845)         \\
\addlinespace
Constant            &       0.741         &      11.799         &       1.173         &      -2.830         &     -13.012         &      19.146         &      -0.487         \\
                    &     (2.428)         &    (10.746)         &     (7.090)         &     (9.029)         &    (24.332)         &    (41.453)         &     (3.633)         \\
\midrule
Obs.                &    3958.000         &     859.000         &     828.000         &     863.000         &     475.000         &     489.000         &     444.000         \\
County Fixed Effects&         yes         &         yes         &         yes         &         yes         &         yes         &         yes         &         yes         \\
$R^2$                 &       0.281         &       0.500         &       0.444         &       0.445         &       0.469         &       0.439         &       0.549         \\
\bottomrule
\multicolumn{8}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{8}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.010\)}\\
\end{tabular}
\end{table}


==> tables/robustness/first_stage_days80.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{First Stage estimates of High Heat Days (80 Degrees) as an instrument for Return to Farming}
\begin{tabular}{l*{5}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
days\_count          &                     &                     &                     &                     &                     \\
                    &                     &                     &                     &                     &                     \\
\addlinespace
Farm Return         &                     &                     &                     &                     &                     \\
                    &                     &                     &                     &                     &                     \\
\addlinespace
Median Census Age   &       0.002         &      -0.002         &       0.008         &      -0.012         &       0.007         \\
                    &     (0.004)         &     (0.018)         &     (0.009)         &     (0.008)         &     (0.008)         \\
\addlinespace
Unemployment Rate   &       0.005\sym{*}  &       0.002         &       0.009         &      -0.000         &       0.002         \\
                    &     (0.003)         &     (0.012)         &     (0.007)         &     (0.006)         &     (0.007)         \\
\addlinespace
High Heat Days      &      -0.005\sym{***}&      -0.006\sym{***}&      -0.002\sym{**} &      -0.006\sym{***}&      -0.003\sym{***}\\
                    &     (0.000)         &     (0.001)         &     (0.001)         &     (0.001)         &     (0.001)         \\
\addlinespace
Constant            &       6.391\sym{***}&       6.602\sym{***}&       6.079\sym{***}&       7.066\sym{***}&       6.144\sym{***}\\
                    &     (0.167)         &     (0.847)         &     (0.362)         &     (0.365)         &     (0.336)         \\
\midrule
Obs.                &    3958.000         &     475.000         &     863.000         &    1348.000         &    1272.000         \\
County Fixed Effects&         yes         &         yes         &         yes         &         yes         &         yes         \\
Year Fixed Effects  &                     &                     &                     &                     &                     \\
$R^2$                 &       0.908         &       0.934         &       0.945         &       0.923         &       0.930         \\
\bottomrule
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{6}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.010\)}\\
\end{tabular}
\end{table}


==> tables/robustness/first_stage_days86.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{First Stage estimates of High Heat Days (86 Degrees) as an instrument for Return to Farming}
\begin{tabular}{l*{5}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}         &\multicolumn{1}{c}{(5)}         \\
\midrule
days\_count          &                     &                     &                     &                     &                     \\
                    &                     &                     &                     &                     &                     \\
\addlinespace
Farm Return         &                     &                     &                     &                     &                     \\
                    &                     &                     &                     &                     &                     \\
\addlinespace
Median Census Age   &       0.004         &      -0.003         &       0.010         &      -0.008         &       0.009         \\
                    &     (0.004)         &     (0.018)         &     (0.009)         &     (0.009)         &     (0.008)         \\
\addlinespace
Unemployment Rate   &       0.004         &      -0.002         &       0.011         &      -0.002         &       0.001         \\
                    &     (0.003)         &     (0.012)         &     (0.007)         &     (0.006)         &     (0.007)         \\
\addlinespace
days\_count86        &      -0.005\sym{**} &      -0.022\sym{***}&       0.002         &      -0.003         &       0.003         \\
                    &     (0.002)         &     (0.005)         &     (0.005)         &     (0.004)         &     (0.004)         \\
\addlinespace
Constant            &       6.224\sym{***}&       6.494\sym{***}&       5.924\sym{***}&       6.830\sym{***}&       6.035\sym{***}\\
                    &     (0.169)         &     (0.846)         &     (0.357)         &     (0.374)         &     (0.339)         \\
\midrule
Obs.                &    3958.000         &     475.000         &     863.000         &    1348.000         &    1272.000         \\
County Fixed Effects&         yes         &         yes         &         yes         &         yes         &         yes         \\
Year Fixed Effects  &                     &                     &                     &                     &                     \\
$R^2$                 &       0.905         &       0.935         &       0.945         &       0.918         &       0.929         \\
\bottomrule
\multicolumn{6}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{6}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.010\)}\\
\end{tabular}
\end{table}

